Rising Rested Bandits: Lower Bounds and Efficient Algorithms

This paper is in the field of stochastic Multi-Armed Bandits (MABs), i.e. those sequential selection techniques able to learn online using only the feedback given by the chosen option (a.k.a. $arm$). We study a particular case of the rested bandits in which the arms' expected reward is monotonically non-decreasing and concave. We study the inherent sample complexity of the regret minimization problem by deriving suitable regret lower bounds. Then, we design an algorithm for the rested case $\textit{R-ed-UCB}$, providing a regret bound depending on the properties of the instance and, under certain circumstances, of $\widetilde{\mathcal{O}}(T^{\frac{2}{3}})$. We empirically compare our algorithms with state-of-the-art methods for non-stationary MABs over several synthetically generated tasks and an online model selection problem for a real-world dataset

==> tikz/plots/firstlb.tex <==
\begin{figure}[!ht]
\centering
\resizebox{1\textwidth}{!}{%
\begin{circuitikz}[scale=0.8] % Added scale=0.8 to adjust the size of the diagram
\tikzset{every node/.append style={font=\normalsize}} % Changed \tikzstyle to \tikzset
\draw [->, >=Stealth] (2.5,3.5) -- (2.5,14.5) node[pos=1,left]{$\mu(t)$}; % Changed \tikzstyle to \tikzset
\draw [->, >=Stealth] (2.5,3.5) -- (16.5,3.5) node[pos=0.5,below]{$\textit{pulls t}$}; % Corrected the closing curly brace and removed unnecessary 't'
\draw [short] (2.5,3.5) -- (7.5,7.25);
\draw [short] (7.5,7.25) -- (16.25,7.25)node[pos=1,right, fill=white]{$\textit{first instance}$}; % Corrected the closing curly brace
\draw [short] (7.5,7.25) -- (16.25,13.5)node[pos=1,right, fill=white]{$\textit{second instance}$}; % Corrected the closing curly brace
\draw [ color={rgb,255:red,223; green,12; blue,12}, dashed] (2.5,8.5) -- (16.5,8.5)node[pos=0.9,below, fill=white]{$\textit{rewards average up to T for the second instance}$};
\draw [ color={rgb,255:red,223; green,12; blue,12}, dashed] (2.5,6.5) -- (16.25,6.5)node[pos=0.9,below, fill=white]{$\textit{rewards average up to T for the first instance}$};
\draw [ color={rgb,255:red,86; green,12; blue,223}, <->, >=Stealth] (2.25,6.5) -- (2.25,8.5)node[pos=0.5,left, fill=white]{$2\overline{\Delta}$}; % Removed unnecessary \textit{} and escaped the math mode
\draw [ color={rgb,255:red,86; green,12; blue,223}, short] (2.5,7.5) -- (16.25,7.5)node[pos=0.2,above, fill=white]{$\textit{fixed arm}$}; % Corrected the closing curly brace
\draw [ color={rgb,255:red,86; green,12; blue,223}, <->, >=Stealth] (3.5,7.5) -- (3.5,8.5)node[pos=0.5,left]{$\overline{\Delta}$}; % Removed unnecessary \textit{} and escaped the math mode
\draw [ color={rgb,255:red,86; green,12; blue,223}, <->, >=Stealth] (3.5,6.5) -- (3.5,7.5)node[pos=0.5,left]{$\overline{\Delta}$}; % Removed unnecessary \textit{} and escaped the math mode
\draw [dashed] (7.5,7.25) -- (7.5,3.5);
\draw [<->, >=Stealth] (2.5,4) -- (7.5,4)node[pos=0.65,left, fill=white]{$\textit{cT}$};
\draw [<->, >=Stealth] (7.5,4) -- (16.25,4)node[pos=0.65,left, fill=white]{$\textit{c'T}$};
\end{circuitikz}
}%
\caption{The two two armed bandits instances}
\label{fig:my_label}
\end{figure}

==> tikz/plots/lblogistic.tex <==
\begin{figure}[!ht]
\centering
\resizebox{1\textwidth}{!}{%
\begin{circuitikz}[scale=0.8] % Added scale=0.8 to adjust the size of the diagram
\tikzset{every node/.append style={font=\normalsize}} % Changed \tikzstyle to \tikzset
\draw [->, >=Stealth] (0,3) -- (0,12.5) node[pos=1,left, fill=white]{$\mu(t)$}; % Changed \tikzstyle to \tikzset
\draw [->, >=Stealth] (0,3) -- (14,3) node[pos=0.5,below]{$\textit{pulls t}$}; % Corrected the closing curly brace and removed unnecessary 't'
\draw [short] (0,3) .. controls (10,3.5) and (2.5,11.25) .. (12.5,11.75) node[pos=1,right, fill=white]{$\textit{first instance}$}; % Corrected the closing curly brace
\draw [short] (5.75,6) -- (12.5,6) node[pos=1,right, fill=white]{$\textit{first instance}$}; % Corrected the closing curly brace
\draw [dashed] (5.75,6) -- (5.75,3);
\draw [<->, >=Stealth] (5.75,6) -- (0,6) node[pos=0.5, fill=white]{$\textit{cT}$};
\draw [ color={rgb,255:red,0; green,0; blue,255}, short] (0,6.75) -- (12.5,6.75) node[pos=0.25,above]{$\textit{fixed arm}$}; % Corrected the closing curly brace
\draw [ color={rgb,255:red,255; green,0; blue,0}, dashed] (0,7.75) -- (12.5,7.75) node[pos=0.90,below]{$\textit{rewards average second instance}$}; % Corrected the closing curly brace
\draw [ color={rgb,255:red,255; green,0; blue,0}, dashed] (0,5.75) -- (12.5,5.75) node[pos=0.90,below, fill=white]{$\textit{rewards average first instance}$}; % Corrected the closing curly brace
\draw [ color={rgb,255:red,0; green,0; blue,255}, <->, >=Stealth] (-0.25,5.75) -- (-0.25,7.75) node[pos=0.5,left]{$2\Delta$}; % Removed unnecessary \textit{} and escaped the math mode
\draw [ color={rgb,255:red,0; green,0; blue,255}, <->, >=Stealth] (1.25,5.75) -- (1.25,6.75) node[pos=0.5,left]{$\Delta$}; % Removed unnecessary \textit{} and escaped the math mode
\draw [ color={rgb,255:red,0; green,0; blue,255}, <->, >=Stealth] (1.25,6.75) -- (1.25,7.75) node[pos=0.5,left]{$\Delta$}; % Removed unnecessary \textit{} and escaped the math mode
\draw [ color={rgb,255:red,0; green,255; blue,128}, dashed] (5.75,6) -- (12.5,10.75) node[pos=0.90,right,fill=white]{$\textit{under estimation}$}; % Corrected the closing curly brace
\draw [<->, >=Stealth] (5.75,4.25) -- (12.5,4.25) node[pos=0.5, fill=white]{$\textit{c'T}$};
\end{circuitikz}
}%
\caption{General Rising}
\label{fig:my_label}
\end{figure}
